Hercules Against Data Series Similarity Search

We propose Hercules, a parallel tree-based technique for exact similarity search on massive disk-based data series collections. We present novel index construction and query answering algorithms that leverage different summarization techniques, carefully schedule costly operations, optimize memory and disk accesses, and exploit the multi-threading and SIMD capabilities of modern hardware to perform CPU-intensive calculations. We demonstrate the superiority and robustness of Hercules with an extensive experimental evaluation against state-of-the-art techniques, using many synthetic and real datasets, and query workloads of varying difficulty. The results show that Hercules performs up to one order of magnitude faster than the best competitor (which is not always the same). Moreover, Hercules is the only index that outperforms the optimized scan on all scenarios, including the hard query workloads on disk-based datasets. This paper was published in the Proceedings of the VLDB Endowment, Volume 15, Number 10, June 2022.

==> discussion.tex <==
\section{Discussion}

\label{sec:discussion}

In the data series literature, competing similarity search methods have never been compared together under a unified experimental scheme.
The objective of this experimental evaluation is to consolidate previous work on data series whole-matching similarity search and prepare a solid ground for further developments in the field.
% Despite the fact that the tasks involved to ensure a fair and thorough comparison proved to be difficult and time consuming.

We undertook a challenging and laborious task, where we re-implemented from scratch three algorithms: iSAX2+, SFA trie, and DSTree, and optimized memory management problems (swapping, and out-of-memory errors) in R*-tree, M-tree, and Stepwise.
%all methods, except for ADS+, UCR Suite, and MASS.
Choosing C/C++ provided considerable performance gains, but also required low-level memory management optimizations.
We believe the effort involved was well worth it since the results of our experimental evaluation emphatically demonstrate the importance of the experimental setup on the relative performance of the various methods.
%In fact, it is of paramount importance that for each method the following 6 rules are followed: a) same programming language used, b) the parameters are fine-tuned, c) the experiments are run on the same hardware and software platform, d) the type and size of the query workload is varied, e) both in-memory and out-of-memory datasets are used, and f) all relevant optimization techniques are applied.
To further facilitate research in the field we publicize our source code and experimental results~\cite{url/DSSeval}.
%Thanks to this work, we are now able to discriminate the real value of each method, its strengths and weaknesses.
% Our study brings to the forefront one relatively old technique, the DSTree, which thanks to its data-adaptive summarization (and our optimized implementation) wins over competing methods in many scenarios.
This section summarizes the lessons learned in this study.

\noindent{\bf Unexpected Results.}
%Before running experiments with the Stepwise method, we expected it to be competitive with the other approaches, particularly since it was reported to surpass sequential scan and iSAX~\cite{conf/kdd/Karras2011}.
For some of the algorithms our experimental evaluation revealed some unexpected results.

(1) \emph{The Stepwise method performed lower than our expectations.}
This was both due to the fact that our baseline sequential scan was fully optimized for early abandoning and computation optimization, but most importantly because of \emph{a different experimental setup}.
The original implementation of Stepwise performed batched query answering.
In our case we compared all methods on single query at a time workload scenario.
This demonstrates the importance of \emph{the experimental setup and workload type}.

(2) \emph{For exact queries on out-of-memory data on the HDD machine, ADS+ is underperforming.}
The reason is that ADS+ performs multiple skips while pruning at a per series level and is thus significantly affected by the hard disk's latency.
In the original study~\cite{journal/vldb/Zoumpatianos2016}, ADS+ was run on a machine with 60\% of the hard disk throughput of the one used in the current work.
The HDD setup with the 6 RAID0 disks gave a significant advantage on methods that perform sequential scans on larger blocks of data and less skips. On the SDD machine, however, the trend is reversed, and ADS+ becomes the best contender overall.
These observations demonstrate the importance of \emph{the hardware setup}. 

(3) \emph{The optimal parameters of most algorithms were different than the ones presented in their respective papers.} 
This is because some methods were not tuned before: the iSAX2+, DSTree and SFA papers have no tuning experiments. We tuned each for varying leaf and buffer sizes (due to lack of space, we only reported results for leaf parameterization in Figure~\ref{fig:exact:leafsize:time:idxproc}; buffer tuning experiments can be found in our archive~\cite{url/DSSeval}). For SFA, we also tuned the sample size used to identify the breakpoints, binning method (equi-depth vs. equi-width), and number of symbols used for the SFA discretization. 
Another reason is that we studied in more detail methods that were partially tuned (e.g., ADS+ was tuned only for varying leaf size; we also varied the buffer size and found that, allowing most of RAM to buffering hurts performance), as well the same methods on different hardware (e.g., our leaf size experiments on the SSD machine resulted to optimal leaf thresholds an order of magnitude smaller than the ones on the HDD machine). 
These findings further demonstrate the need for \emph{careful parameter-tuning}.

%In the next paragraph, we discuss in further detail the TLB resutls which also countered our expectations. 
(4) \emph{The quality of the summarization, as measured by TLB and pruning, is not necessarily correlated to time performance.} 
This stresses the importance of algorithms and implementations and their dependence on hardware.
For example, ADS+ achieves very high pruning, yet, in terms of time it is outperformed by other methods.
While summarization quality is an important factor on its own, it is of crucial importance to 
%carefully design algorithms that 
be considered alongside 
%access patterns and hardware characteristics.
the properties of the index structure and the hardware platform.
%For example, the ratio between latency (random access) and throughput (sequential access) is an important factor that can guide such decisions.


\noindent{\bf Speed-up Opportunities.}
Through our analysis, we identified multiple factors that affect performance for all the methods examined. 
In turn, these factors reveal opportunities and point to directions for performance improvements.

(1) \emph{Stepwise} offers many such avenues.
Its storage scheme could be optimized to reduce the number of random I/O during query answering, and its query answering algorithm would benefit a lot from parallelization and modern hardware optimizations (i.e., through multi-core and SIMD parallelism), as 50\%-98\% of total time is CPU. 

(2) \emph{DSTree} is very fast at query answering, but rather slow at index building.
Nevertheless, a large percentage of this time (85-90\%) is CPU. 
%(ranging from 89\% for the 25GB dataset to 84\% for  the 1TB dataset). 
Therefore, also the indexing performance of DSTree can be improved by exploiting modern hardware. 
Moreover, bulk loading during indexing, and buffering during querying, would also make it even faster.

(3) A similar observation holds for \emph{MASS}.
Even though this method is not designed for whole-matching data series similarity search, its performance can be significantly enhanced with parallelism and modern hardware exploitation, since 90\% of its execution time is CPU cost.

(4) %Finally, we confirmed the strengths of the \emph{ADS+} algorithm:
%%, which is the state-of-the-art data series index:
%fast index building, which enables it to answer the first query much faster than the other index methods, and indexing and query answering on SSD platforms.
%%and to answer \textbf{??? (x number of ) ???} queries before the other approaches have finished the index building phase.
%We identified an additional scenario where ADS+ is clearly the overall winner, that is, whole-matching similarity search for long data series.
Finally, we obtained a better understanding of the \emph{ADS+} algorithm. 
Apart from being very fast in index building, our results showed that it also has a leading performance for whole-matching similarity search for \emph{long} data series.
We also discovered that the main bottleneck for 
%our index and issued some recommendations for future improvements.
ADS+ are the multiple skips performed during query answering.
Its effects could be masked by controlling the size of the data segments skipped (i.e., skipping/reading large continuous blocks), and through asynchronous I/O.
Moreover, because of its very good pruning power (that leads to an increased number of skips), we expect ADS+ to work well whenever random access is cheap, e.g., with SSDs and main-memory systems.

\noindent{\bf Data-adaptive Partitioning.}
While the SFA trie and iSAX-based index building algorithms are much faster than the DSTree index building algorithm, their performance during query answering is much worse than that of DSTree.
DSTree spends more time during indexing, intelligently adapting its leaf summarizations when split operations are performed.
This leads to better data clustering and as a result faster query execution.
On the contrary, both iSAX and SFA have fixed maximum resolutions, and iSAX indexes can only perform splits on predefined split-points.
Even though iSAX summarizations at full resolution offer excellent pruning power (see ADS+ in Figures~\ref{fig:exact:synthetic:datasize:pruning:combined},~\ref{fig:exact:synthetic:length:pruning:combined},~\ref{fig:exact:real:pruning:combined}), grouping them using fixed split-points in an iSAX-based index does not allow for effective clustering (see Figure \ref{fig:exact:datasize:fill:combined}).
This is both an advantage, as indexing and approximate query answering are extremely fast, but also a drawback as it does not allow clustering to adapt to the distribution of the dataset.

\noindent{\bf Approximate Query Answering.} Approximate answers provide a viable alternative when exact solutions are not required, with many methods having a small effective error and great performance (Figures \ref{fig:exact:synthetic:datasize:error:combined}-\ref{fig:exact:real:error:combined}). 
A detailed evaluation of approximate methods is part of our future work.

\noindent{\bf Access-Path Selection.}
Finally, our results demonstrate that the pruning ratio, along with the ability of an index to cluster together similar data series in large contiguous blocks of data, is crucial for its performance. 
Moreover, our results confirm the intuitive result that the smallest the pruning ratio, the highest the probability that a sequential scan will perform better than an index, as can be observed for the hard queries in Table~\ref{tab:summary}. 
This is because it will avoid costly random accesses patterns on a large part of the dataset. 
However, the decision between a scan or an index, and more specifically, the choice of an index, is not trivial, but is based on a combination of factors: (a) the effectiveness of the summarization used by the index (which can be estimated by the pruning ratio); 
%to accurately represent data series, as this dictates the pruning ratio (i.e., the amount of data that have to be accessed), 
(b) the ability of the index to cluster together similar data series (which determines the access pattern);
%this dictates the access pattern (i.e., the number of seeks performed or how the data are accessed), 
and (c) the hardware characteristics (which dictate the data access latencies).
%properties like throughput and latency, as they dictate the cost of a random seek vs a sequential scan (i.e., how much of an overhead a random access is). 
%Being able to make the right choice on which index to build and when to use it, depends not only on the index itself, but also on the query workload and the current hardware, thus raising an interesting optimization problem, which has never been studied in the past in the domain of data series similarity search. Further exploration of this topic is part of our future work.
This context gives rise to interesting optimization problems, which have never before been studied in the domain of data series similarity search.



==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Before presenting the workflow of Hercules, we will first give an overview of the the SAX summarization, and the Stepwise and DSTree methods. 

\subsection{SAX}
\label{subsec:sax}

The {\it Symbolic Aggregate Approximation} (SAX)~\cite{conf/dmkd/LinKLC03} first transforms a vector $V$ using the {\it Piecewise Aggregate Approximation} (PAA)~\cite{journal/kais/Keogh2001}. The PAA summarization divides $V$ into $l$ equi-length segments and represents each segment with one floating-point value corresponding to the mean of all the points belonging to the segment (Fig.~\ref{fig:paa}). SAX reduces the footprint of the PAA representation by applying a discretization technique that map PAA values to a discrete set of symbols (alphabet) that can be succinctly represented in binary form.
%The discretization uses a heuristic to place $b$ breakpoints on the y-axis. If we draw lines parallel to the x-axis and passing through each of the breakpoints, we can see that the space is divided into $a$ regions where $a = b+1$. Each region is labeled using a discrete alphabet of size $a$, $a$ is also called the cardinality of SAX. The $y_i$ of each dimension $C_i$ is then mapped to a discrete value from this alphabet. 
A SAX representation consists of $l$ such symbols.
An $i$SAX (indexable SAX)~\cite{conf/kdd/Shieh2008} representation can have an arbitrary alphabet size for each segment (Fig.~\ref{fig:sax}).
%. and each symbol is represented using the same cardinality, that is the alphabet size is fixed. The iSAX technique extends SAX to allow comparisons of SAX representations of different cardinality, which in turn makes SAX indexable. An iSAX word is represented using a higher resolution by adding a breakpoint on the y-axis. The higher resolution word will also consist of $l$ symbols but the alphabet size available for a given symbol will be larger.  The maximum resolution of a SAX word uses the maximum alphabet size which is 256.

\begin{figure}[!htb]
	\captionsetup{justification=centering}
	\captionsetup[subfigure]{justification=centering}
	\centering
	\begin{subfigure}{0.6\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{vector.pdf}
	\end{subfigure}
	\begin{subfigure}{0.45\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{paa_v3.pdf}
		\caption{PAA}
		\label{fig:paa}
	\end{subfigure}
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{sax_v3.pdf}
		\caption{SAX}
		\label{fig:sax}
	\end{subfigure}
	\caption{The PAA and SAX representations}
	\label{fig:paa-sax}
\end{figure}


\subsection{DSTree}


The DSTree~\cite{conf/vldb/Wang2013} approach uses the {\it Extended Adaptive Piecewise Approximation} (EAPCA)~\cite{conf/vldb/Wang2013}, which extends the {\it Adaptive Piecewise Constant Approximation} (APCA)~\cite{journal/acds/Chakrabarti2002} by using more information to represent each segment of a vector $V$. The APCA segmentation divides $V$ into $l$ varying-length segments and represents each segment using the mean value of the points belonging to it (Fig~\ref{fig:apca}). The EAPCA representation uses the standard deviation in addition to the mean to represent each segment (Fig~\ref{fig:eapca}). 


\begin{figure}[!htb]
	\captionsetup{justification=centering}
	\captionsetup[subfigure]{justification=centering}
	\centering
	\begin{subfigure}{0.45\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{apca_v3.pdf}
		\caption{APCA}
		\label{fig:apca}
	\end{subfigure}
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{eapca_v3.pdf}
		\caption{EAPCA}
		\label{fig:eapca}
	\end{subfigure}
	\caption{The APCA and EAPCA representations}
	\label{fig:paa-sax}
\end{figure}

The DSTree intertwines segmentation and indexing, building an unbalanced binary tree with two types of nodes: internal nodes and leaf nodes. Each node contains: 1) the number of vectors indexed at its subtree; 2) the segmentation {\bf \textit{SG}} at this node indicated by the the right endpoints of each segment; and 3) a synopsis $Z = (z_1, z_2, ..., z_m), where *\ z_i = \{\mu_{min}, \mu_{max}, \rho_{min}, \rho_{max}\}$ that contains, for each segment, the minimum and maximum means and standard deviations of all series indexed at this node. A leaf node is associated with a filename on disk that stores all its vectors. All leaves have a maximum capacity of $\psi$ vectors, called the leaf threshold, i.e., each leaf can store a maximum of $\psi$ vectors. An internal node contains pointers to the left and right children nodes and a splitting policy. Figure ~\ref{fig:dstree-tree} shows a sample DSTree binary tree. 


\begin{figure}[!htb]
	\captionsetup{justification=centering}
	\captionsetup[subfigure]{justification=centering}
	\centering
	\includegraphics[width=0.8\columnwidth]{dstree_tree_v2.pdf}
	\caption{A sample binary tree index created by the DSTree}
	\label{fig:dstree-tree}
\end{figure}

The dynamic segmentation allows the DSTree to summarize a data series more accurately than the other dimensionality reduction techniques. It is exploited in the node splitting algorithm by allowing the resolution of a summarization to increase along two dimensions: vertically and horizontally.
%, unlike the other data series indexes which allow either one or the other. 
(Instead, 
SAX-based indexes allow horizontal splitting by adding a breakpoint to the y-axis) 
In addition to a lower bounding distance, the DSTree also supports an upper bounding distance.  It uses both distances to determine the optimal splitting policy for each node. 
The data series in a given node are all segmented using the same policy but each node has its own segmentation policy which may result in nodes having a different number of segments or segments of different lengths.

Figure~\ref{fig:dstree-indexing-answering-workflow} summarizes the workflow of DSTree's index building algorithm. The algorithm loads the dataset into memory one vector at a time, reading sequentially form the original file. Each loaded vector is inserted into the tree traversing the index to find the appropriate leaf, routing left or right depending on the split policy of the visited node, and updating the synopsis of all traversed nodes. Each Leaf points to a FileBuffer which itself points to a BufferedList that contains the data stored in the leaf and currently present in-memory.  Each leaf is associated with a file on disk. FileBuffers are organized in a Hash Map called the FileMap. The FileMap contains <key,value> pairs where each pair is an index corresponding to a leaf’s Filename and the value is a pointer to the FileBuffer of the leaf. 

Once memory is full, half of the FileBuffers are flushed into disk, each vector is stored in the file corresponding to the leaf where it was stored. In the final flush, The index tree and the data remaining in memory is flushed to disk.

\begin{figure}[!htb]
	\includegraphics[width=\columnwidth] {dstree_workflow_v2}
	\caption{DSTree Indexing Workflow}  
	\label{fig:dstree-indexing-answering-workflow}
\end{figure}

